Towards Understanding Hierarchical Learning: Benefits of Neural Representations

Deep neural networks can empirically perform efficient hierarchical learning, in which the layers learn useful representations of the data. However, how they make use of the intermediate representations are not explained by recent theories that relate them to "shallow learners" such as kernels. In this work, we demonstrate that intermediate neural representations add more flexibility to neural networks and can be advantageous over raw inputs. We consider a fixed, randomly initialized neural network as a representation function fed into another trainable network. When the trainable network is the quadratic Taylor model of a wide two-layer network, we show that neural representation can achieve improved sample complexities compared with the raw input: For learning a low-rank degree-$p$ polynomial ($p \geq 4$) in $d$ dimension, neural representation requires only $\tilde{O}(d^{\lceil p/2 \rceil})$ samples, while the best-known sample complexity upper bound for the raw input is $\tilde{O}(d^{p-1})$. We contrast our result with a lower bound showing that neural representations do not improve over the raw input (in the infinite width limit), when the trainable network is instead a neural tangent kernel. Our results characterize when neural representations are beneficial, and may provide a new perspective on why depth is important in deep learning.

==> Sections_arxiv/neural-reps-june-2.tex <==
\section{Learning with neural representations}
\label{sec:upperbound}

\subsection{Improved Sample Complexity using Neural Representations}
\label{section:neural-reps}
We formally present how learning with neural representations yields
better generalization and reduces sample complexity. We compete
\quadneural~with a family of polynomials for replicating the ground
truth mapping between the feature $\xb$ and response
$y$. Specifically, we denote
%~\yub{Merge assumption 4 into here.}
\begin{align}
B(r_\star, p_{\max}, A, C) &=\Bigg\{f: f(\xb) = \sum_{s=1}^{r_\star} \alpha_s (\boldsymbol{\beta}_s^\top \xb)^{p_s}, p_s\le p_{\max},\notag\\
&\hspace{1.2in}\sum_{s=1}^{r_\star} \alpha_s^2 \le A,~\max_{1\le s\le r_\star}\EE_{\xb} [(\boldsymbol{\beta}_s^\top \xb)^{2p_s}] \leq C\Bigg\}.\label{B-def}
\end{align}
\yub{Add $C$ as argument along with $(r_\star, p_{\max}, A)$? or make $C=1$ (and then $A$ can blow up but that's fine)?}~\yub{Power should be $2p_s$ in definition of $C$?}
Note that the moment condition in \eqref{B-def} ensures that the polynomial family $B(r_\star, p_{\max}, A, C)$ has a finite radius. In addition, by Jensen's inequality, each polynomial has bounded moments up to order $2p_s$.

We show \quadneural~can efficiently learn any function in $B(r_\star,
p_{\max}, A, C)$. Recall the model with weight parameter $\Wb$ computes
\begin{align*}
  f_{\Wb}(\xb) = \frac{1}{2\sqrt{m}} \sum_{r=1}^m a_{0, r}
  \phi''(\wb_{0, r}^\top \hb(\xb) \ge 0)\left(\wb_r^\top
  \hb(\xb)\right)^2
\end{align*}
with $\hb(\xb) = \hat{\bSigma}^{-1/2} \sigma\left(\Vb \xb + \bbb\right)$.
For simplicity, we take $\phi''(\cdot) = \sigma(\cdot) =
\ind\{\cdot\}$~\yub{TODO(yub): move choice of $\phi$ and $\sigma$ to
  algorithm part}.
We also make the following additional assumptions.
\begin{assumption}[Positive Definitive Covariance]\label{assumption_covariance}
\yub{assumption need not be whp. can say after assumption that
  e.g. this holds whp for uniform x.}
With high probability over the randomness of $\Vb, \bbb$, we have $\lambda_{\min}(\bSigma) \geq c$ for some constant $c$, where $\lambda_{\min}$ denotes the smallest singular value and $\bSigma = \EE_{\xb} [\sigma\left(\Vb \xb + \bbb\right) \sigma\left(\Vb \xb + \bbb\right)^\top]$.
\end{assumption}
Assumption \ref{assumption_covariance} only requires mild conditions on the data distribution. For example, when $\xb$ is uniform on $\SSS^{d-1}$, \cite{ghorbani2019linearized} proved that $\lambda_{\min}(\bSigma) \geq c$ holds with high probability as $d \rightarrow \infty$. 
%\begin{assumption}[Bounded Moments]\label{assumption_moment}
%For any $s = 1, \dots, r_\star$, we have $\EE_{\xb} [(\boldsymbol{\beta}_s^\top \xb)^{p_s}] \leq C$ for some constant $C$.
%\end{assumption}
The following theorem establishes the expressivity of
\quadneural~for approximating any function in $B(r_\star, p_{\max}, A, C)$.
% \yub{Bounded by $(1+\gamma)\opt + \epsilon$ instead?}
\begin{theorem}[Expressivity of \quadneural]
  \label{thm:quadneural_expressivity}
Suppose Assumptions \ref{assumption_input} -- \ref{assumption_covariance} hold. Given any $f_0 \in B(r_\star, p_{\max}, A, C)$, any small $\epsilon, \delta \in (0, 1)$, we choose 
%$$D \geq \frac{2\times 50^2 r_{\star}^3 \sum_{s=1}^{r_\star} (p_s+1)^5 \norm{\boldsymbol{\beta}_s}_2^{2 \lceil p_s/2 \rceil}}{\epsilon^2 \delta} \quad \textrm{and} \quad m \geq \frac{54 r_\star d(1+\log 1/\delta)}{\epsilon^2} \log \frac{1}{\epsilon}.$$
\begin{align*}
& D \leq O\left(\frac{r_{\star}^{7/2} A C^{1/2} \sum_{s=1}^{r_\star} (p_s+1)^5 \norm{\boldsymbol{\beta}_s}_2^{2 \lceil p_s/2 \rceil}}{\epsilon^2 \delta}\right) \quad \textrm{and} \\
& m \geq O\left(\frac{r_\star^{3/2} A C^{1/2} d(1+\log 1/\delta)}{\epsilon^2 \delta} \log \frac{7 A^{1/2} r_\star^{1/4} C^{1/4}}{\epsilon}\right).
\end{align*}
Let $\wb_{0, r} \overset{{\rm iid}}{\sim} \normal(\boldsymbol{0}, \Ib_D)$ and $a_{0, r} \overset{{\rm iid}}{\sim} \textrm{Uniform}\{-1, 1\}$ for $r = 1, \dots, m$, then there exist proper $\{\wb_r^*\}$ such that with probability at least $1 - 3\delta$, we have
\begin{align*}
\norm{\frac{1}{2\sqrt{m}} \sum_{r=1}^m a_{0, r} \mathds{1}\{\wb_{0, r}^\top \hb(\xb) \geq 0\} \left((\wb_r^*)^\top \hb(\xb)\right)^2 - f_0(\xb)}_{L_2} \leq 
%7 A^{1/2} r_\star^{1/4} C^{1/4} \epsilon.
\epsilon.
%\sqrt{A \sum_{s=1}^{r_\star} \norm{(\boldsymbol{\beta}_s^\top \xb)^{p_s}}_{L_2}}.
\end{align*}
\end{theorem}
\yub{again, need $a_r\in\set{\pm 1}$?} \yub{bound of $D$ should have power $2p_s$?}

\begin{theorem}[Sample complexity of learning with \quadneural]
\label{thm:quadneural_generalization}
Suppose Assumptions \ref{assumption_input} -- \ref{assumption_covariance} hold. Given any $f_0 \in B(r_\star, p_{\max}, A)$ and assume for some $\mathsf{OPT} > 0$, we have $\cR(f_0) \leq \mathsf{OPT}$. For any $\epsilon \in (0, 1)$, $\delta \in (0, 1)$ and $\tau = \Theta(1)$, we choose $D$ and $m$ the same as in Theorem \ref{thm:quadneural_expressivity} and proper $\lambda > 0$.
%\begin{align*}
%& D \geq \frac{392\times50^2 r_{\star}^{7/2} A C^{1/2} \sum_{s=1}^{r_\star} (p_s+1)^5 \norm{\boldsymbol{\beta}_s}_2^{2 \lceil p_s/2 \rceil}}{\epsilon^2 \delta} \quad \textrm{and} \\
%& m \geq \frac{49\times54 r_\star^{3/2} A C^{1/2} d(1+\log 1/\delta)}{\epsilon^2} \log \frac{7 A^{1/2} r_\star^{1/4} C^{1/4}}{\epsilon}.
%\end{align*}
Then with probability at least $1-5\delta$ over the randomness of data and initialization, any second-order stationary point $\hat{\Wb}$ of the regularized risk satisfies
\begin{align*}
\hat{\cR}_{\lambda}(f^Q_{\hat{\Wb}}) \leq (1+\tau)(\mathsf{OPT} + \epsilon)+ \epsilon,
\end{align*}
and the generalization error is bounded by
\begin{align*}
\EE_{\Wb_0, \ab_0}\left[\cR(f^Q_{\hat{\Wb}}) -
  \hat{\cR}(f^Q_{\hat{\Wb}})\right] \leq \tilde{O}\left(\sqrt{\lambda_{\min}^{-1}(\bSigma)A^2 C^{3/2} r_{\star}^{9/2}} \frac{\sqrt{\sum_{s=1}^{r_\star} (p_s +1)^5 \norm{\boldsymbol{\beta}}_2^{2\lceil p_s / 2\rceil}}}{\epsilon \sqrt{n}}\right).
% \lambda_{\min}^{-1}(\bSigma)
\end{align*}
\end{theorem}
\yub{make excess risk $\epsilon$ as opposed to $CAr_\star\epsilon$,
  which requires redefining $\epsilon$, and adjust generalization
  error accordingly.}
{\color{blue} Implications of Theorem
  \ref{thm:quadneural_generalization}.}
% \subsection{Warm-up: $r_\star=1$}
% To warm up, we first analyze for $r_\star = 1$ and assume the exponent $p$
% is even.

%\subsection{Motivating example: exact sphercial harmonics as features}
%Take $h(x)$ to be spherical harmonics up to degree $k$. This is
%$O(d^k)$ features whose span contains all degree $\le k$ polynomials
%(exactly).
%
%No need to whiten. Also no need to turn shell to sphere? \yub{If high
%  $k$ does not work, fine to present only $k=2$.}
%\begin{theorem}
%  Generalization error of learning a function in $B(r_\star, p_{\max},
%  A)$ is $O(d^{p_{\rm max}/2}/\epsilon^2)$.
%\end{theorem}
To better interpret Theorem \ref{thm:quadneural_generalization}, we instantiate the error bound to a specific polynomial class $B(r_\star, p_{\max}, 1, 1)$ with $\norm{\boldsymbol{\beta}_s}_2 = O(\sqrt{d})$ for $s = 1, \dots, r_{\star}$. The moment condition \eqref{B-def} is valid for many standard distributions on $\SSS^{d-1}$, e.g., the uniform distribution. To achieve comparable performance with $f_0 \in B(r_\star, p_{\max}, 1, 1)$, we require the generalization error of $f_{\hat{\Wb}}$ bounded by $\epsilon$, which in turn gives rise to $\cR(f_{\hat{\Wb}})^Q \leq (1+\tau) \mathsf{OPT}+2\epsilon$ holds with high probability $1-\delta$. To this end, the required sample complexity grows in the order $$\tilde{O}\left(\frac{d^{\lceil p_{\max} / 2\rceil}}{\epsilon^4} \textrm{poly}(r_\star, \delta^{-1})\right).$$
We compare with the sample complexities of \ntkraw~and \quadraw, which scale as\footnote{We neglect the polynomial dependence on $r_\star$ and $\delta^{-1}$.} $\tilde{O}(d^{p_{\max}} / \epsilon^2)$ \citep{arora2019fine, cao2019generalization} and $\tilde{O}(d^{p_{\max} - 1} / \epsilon^2)$ \citep{bai2019beyond}, respectively. As can be seen, our result largely reduces the dependence on the data dimension $d$ when $p_{\max} \geq 4$. This is a visible improvement, since in modern real-world applications, the data dimension is often very high, e.g. RGB image of resolution $384 \times 384 \times 3$ in ImageNet data set \citep{deng2009imagenet}.

The improved sample complexity stems from two benefits brought by neural representations: 1) Neural representation adapts to the underlying data distribution. Whitening using the estimated covariance matrix essentially incorporates the data information into neural representations. This is in the same spirit as batch normalization \citep{ioffe2015batch}. The difference is that batch normalization is applied entrywise to the input features. Besides, whitening makes neural representations approximately isotropic, which can potentially reduce feature redundancy. 2) Neural representation increases flexibility of the learning model. \quadneural~can be viewed as the Taylor expansion of a three-layer neural network, where only the weights in the middle layer are optimized. With the additional layer, \quadneural~reduces the learning of a high-degree polynomial into learning two low-degree polynomials. In more detail, the intermediate neural representation (first two layers) learns a $p_{\max}/2$-degree polynomial and the third layer further boosts the $p_{\max}/2$-degree polynomial to $p_{\max}$-degree. This makes the whole learning process much easier and more efficient. We believe this perspective throws light on the importance of depth in deep learning and makes important steps towards understanding hierarchical learning.

\subsection{Technical overview}
We highlight essential technical ingredients to establish Theorem \ref{thm:quadneural_expressivity} and \ref{thm:quadneural_generalization}. The complete proof is provided in Appendix \ref{pf:thmquadneural}.

$\bullet$ {\it Expressivity of neural representation}. Our neural representation function $\hb$ is constructed from whitening random features consisting of indicators. It is well known that random indicator features are universal approximators --- can express a large class of general functions. Here we specialize to approximate polynomials.

$\bullet$ {\it Connecting \quadneural~with polynomial family $B(r_\star, p_{\max}, A, C)$}. We show \quadneural~can approximate any function $f_0$ in $B(r_\star, p_{\max}, A, C)$. The \quadneural~model raises any linear combination of neural representation $\hb$ to a power of $2$. We leverage such structural information. Specifically, the neural representation can express a $\lceil p / 2\rceil$-degree polynomial. Then QuadNTK boosts it to a $p$-degree polynomial. Meanwhile, we show that the randomly initialization part in \quadneural~concentrates around a constant. In this way, \quadneural~reproduces each polynomial term in $f_0$.

$\bullet$ {\it Approximate isotropicity}. Whitening plays an important role in improving the sample complexity by forcing the representation $\hb$ nearly isotropic. This is quantified by $M_{h, \textrm{op}}$. In general, for a highly correlated feature vector, $M_{h, \textrm{op}}$ is $O(1)$. However, we show $M_{h, \textrm{op}} = O(1/\sqrt{D})$ with high probability. This reduces the generalization gap by a $\sqrt{D}$ factor.

$\bullet$ {\it Covariance estimation}. We use separate samples to estimate the covariance matrix of the neural representation. This ensures the estimated covariance is independent of the samples used in learning. Doing so sacrifices sample complexity, nonetheless, we show the number of samples required to achieve a good generalization overwhelms that for the covariance estimation.

%We sketch the proof of Theorem \ref{thm:quadneural_expressivity} and Theorem \ref{thm:quadneural_generalization}. The detailed proof is postponed to Appendix \ref{pf:thmquadneural}.
%
%{\it Proof Sketch of Theorem \ref{thm:quadneural_expressivity}}. The proof is constructive. For a clear exposition, we let $r_{\star} = 1$ and drop the subscript in $p_{\max}$. We also assume $p$ is even and $\alpha > 0$. We first show that with high probability, there exists $\boldsymbol{\theta}$ satisfying $\EE_{\xb}[\boldsymbol{\theta}^\top \hb(\xb) - (\boldsymbol{\beta}^\top\xb)^{p/2}]^2 \leq \epsilon$. This result holds true, since $\hb(\xb)$ is essentially random features capable of representing any polynomials. In more detail, built upon {\it Lemma A.6} in \citet{allen2019learning}, we prove that there exists a function $a(\vb, b)$ satisfying
%\begin{align*}
%\EE_{\vb, b} [a(\vb, b) \ind\{\vb^\top \xb + b \geq 0\}] = (\boldsymbol{\beta}^\top \xb)^{p/2},
%\end{align*}
%where $\vb, b$ are standard Gaussian. By choosing $D = \tilde{O}(d^{p/2}/\epsilon^2)$ and invoking Chebyshev's inequality, we check that $\boldsymbol{\theta} = \frac{1}{D} \hat{\bSigma}^{1/2}[a(\vb_1, b_1), \dots, a(\vb_D, b_D)]^\top$ satisfies $\EE_{\xb}[\boldsymbol{\theta}^\top \hb(\xb) - (\boldsymbol{\beta}^\top\xb)^{p/2}]^2 \leq \epsilon$. Given $\boldsymbol{\theta}$, we choose $\Wb^* = [\wb^*_1, \dots, \wb^*_m]^\top$ with identical rows $\wb_i^* = \sqrt{2\alpha} m^{-1/4} \boldsymbol{\theta}$. Substituting into $f_{\Wb^*}$, we have
%\begin{align*}
%\sqrt{\EE_{\xb}[f_{\Wb^*}(\xb) - f_0(\xb)]^2} = \sqrt{\EE_{\xb}\left[\frac{1}{m}\sum_{r=1}^m 2\alpha \ind\{\wb_{0, r}^\top \hb(\xb)\} (\boldsymbol{\theta}^\top \xb)^2 - \alpha (\boldsymbol{\beta}^\top \xb)^p \right]^2}.
%\end{align*}
%It remains to verify $\frac{1}{m}\sum_{r=1}^m \ind\{\wb_{0, r}^\top \hb(\xb)\}$ well concentrates around its average $1/2$ for sufficiently large $m$. This follows since each $\ind\{\wb_{0, r}^\top \hb(\xb)\}$ is i.i.d. for any fixed $\xb$ and bounded --- thus sub-Gaussian. These arguments proves that $f_{\Wb^*}$ is a close proxy of $f_0$.
%
%{\it Proof Sketch of Theorem \ref{thm:quadneural_generalization}}. Given $\Wb^*$ and Lemmas \ref{lemma:optimization} and \ref{lemma:generalization}, it suffices to bound $B_h$, $B_{w, \star}$ and $M_{h, \textrm{op}}$. $B_h$, $B_{w, \star}$, and $M_{h, \textrm{op}}$ all involve the estimated covariance matrix. To handle this, we replace $\hat{\bSigma}$ with $\bSigma$ by invoking a relative concentration of covariance estimation (Lemma \ref{lemma:covariance_relative}, \citep{vershynin2010introduction}), which implies $0.5\bSigma \preceq \hat{\bSigma} \preceq 1.5\bSigma$ holds with high probability. Then we can derive $\norm{\hb(\xb)}_2^2 = \|\hat{\bSigma}^{-1/2} \bSigma^{1/2} \bSigma^{-1/2} \gb(\xb)\|_2^2 \leq 2 \norm{\bSigma^{-1/2} \gb(\xb)}_2^2$. Under Assumption \ref{assumption_covariance}, we straightforwardly have $\norm{\bSigma^{-1/2} \gb(\xb)}_2^2 \leq c^{-1/2}\sqrt{D}$. This gives rise to a bound on $B_h$. Using the same trick, we can bound $\norm{\Wb^*}_{2, 4}$ and $M_{h, \textrm{op}}$. {\color{blue} polish.}


%\section{Adaptive inputs for quadratic NTK}
%Let $x\in\R^d$ be a raw input with some distribution $P$, and
%\begin{equation*}
%  F(x) \defeq \begin{bmatrix}
%    f_1(x) \\ \vdots \\ f_m(x)
%  \end{bmatrix} \in \R^m
%\end{equation*}
%be a $m$-dimensional feature vector. A primary example is random
%ReLU features: 
%\begin{align*}
%f_i(x) \defeq \sigma(v_i^\top x),~~~{\rm where}~v_i\simiid\normal(0,
%  I_d).
%\end{align*}
%
%We study the norm-based sample complexity for using $F$ to express
%some ground truth function $f_\star(x)$. Define
%\begin{align*}
%  u \defeq \E_{x\sim P}[F(x) f_\star(x)] \in \R^m~~~{\rm and}~~~\Sigma
%  \defeq \E_{x\sim P}[F(x) F(x)^\top] \in\R^{m\times m}.
%\end{align*}
%Assuming $\Sigma \succ 0$, then the optimal $L_2$
%approximation of $f_\star$ is given by
%\begin{align*}
%  \alpha_\star^\top F(x),~~~{\rm where}~\alpha_\star \defeq
%  \Sigma^{-1}u,
%\end{align*}
%which follows from minimizing the following $L_2$ risk over $\alpha\in\R^m$:
%\begin{align*}
%  \E[f_\star(x)^2] - 2\alpha^\top \E[F(x) f_\star(x)] +
%  \alpha^\top \E[F(x) F(x)^\top]\alpha = \E[f_\star(x)^2] -
%  2\alpha^\top u + \alpha^\top \Sigma\alpha^\top.
%\end{align*}
%
%\paragraph{Whitening} Let $\wt{F}(x) = \Sigma^{-1/2}F(x)$ be the
%whitening of $F(x)$, then the optimal $L_2$ approximation of $f_\star$
%is given by
%\begin{align*}
%  \wt{\alpha}_\star^\top \wt{F}(x),~~~{\rm
%  where}~\wt{\alpha}_\star=\Sigma^{-1/2}u.
%\end{align*}
%
%
%\section{Quadratic unfolding}
%
%\begin{lemma}\label{lemma:Q_singular_min}
%  Let $v_1,\dots,v_m\sim {\rm Unif}({\mathbb S}^{d-1})$ be random unit vectors
%  and $Q = [v_1^{\otimes 2},\dots,v_m^{\otimes 2}]\in\R^{d^2\times
%    m}$. When $m\ge O(d^2)$, we have with high probability that
%  \begin{equation*}
%    \sigma_{\min}(Q) \ge O(1).
%  \end{equation*}
%\end{lemma}
%\begin{proof}
%  Proof sketch:
%  \begin{enumerate}
%  \item We have the variational characterization
%    \begin{equation*}
%      \sigma_{d^2}(Q)^2 = \min_{\lfro{A}=1} \sum_{r=1}^m
%      \<v_rv_r^\top, A\>^2
%    \end{equation*}
%  \item Fix any $A\in\R^{d\times d}$ such that $\lfro{A}=1$. Can show
%    the one-sided concentration
%    \begin{equation*}
%      \P\paren{ \frac{1}{m}\sum_{r\le m} (v_r^\top Av_r)^2 \le
%        \frac{c_1}{d^2}\lfro{A}^2 } \le \exp(-c_2m).
%    \end{equation*}
%    This can be done by the ``to indicator'' technique: first find
%    $c_1>0$ such that
%    \begin{equation*}
%      \P_v\paren{ (v^\top Av)^2 \ge \frac{2c_1}{d^2}\lfro{A}^2 } \ge 2/3
%    \end{equation*}
%    holds for all $A$. (We expect this because $\E_v[(v^\top Av)^2]
%    \ge c/d^2\lfro{A}^2$.) Second, we always have the bound
%    \begin{align*}
%      & \quad \P\paren{ \frac{1}{m}\sum_{r\le m} (v_r^\top Av_r)^2 \le
%        \frac{c_1}{d^2}\lfro{A}^2} \le
%        \P\paren{ \#\set{r: (v_r^\top Av_r)^2 \ge
%        \frac{2c_1}{d^2}\lfro{A}^2 } \le m/2} \\
%      & = \P\paren{\frac{1}{m}\sum_{r\le m} \indic{(v_r^\top Av_r)^2 \ge
%        \frac{2c_1}{d^2}\lfro{A}^2} \le 1/2} \le \exp(-c_2m),
%    \end{align*}
%    the last bound following from the Hoeffding inequality for
%    indicators that have expectation at least $2/3$.
%  \item Covering + union bound + Lipschitzness can give the above
%    result uniformly over all $\lfro{A}=1$. The covering number for
%    this set is $\exp(Cd^2)$, so need $m\ge O(d^2)$ for the result to
%    hold w.h.p. over all $A$, i.e.
%    \begin{equation*}
%      \sum_{r\le m} (v_r^\top Av_r)^2 \ge c_1 \cdot
%      \frac{m}{d^2}\lfro{A}^2 \ge O(1).
%    \end{equation*}
%    This is the desired result.
%  \end{enumerate}
%\end{proof}

